Strict Self-Assembly of Discrete Self-Similar Fractal Shapes

This paper gives a (polynomial time) algorithm to decide whether a given Discrete Self-Similar Fractal Shape can be assembled in the aTAM model.In the positive case, the construction relies on a Self-Assembling System in the aTAM which strictly assembles a particular self-similar fractal shape, namely a variant $K^\infty$ of the Sierpinski Carpet. We prove that the aTAM we propose is correct through a novel device, \emph{self-describing circuits} which are generally useful for rigorous yet readable proofs of the behaviour of aTAMs.We then discuss which self-similar fractals can or cannot be strictly self-assembled in the aTAM. It turns out that the ability of iterates of the generator to pass information is crucial: either this \emph{bandwidth} is eventually sufficient in both cardinal directions and $K^\infty$ appears within the fractal pattern after some finite number of iterations, or that bandwidth remains ever insufficient in one direction and any aTAM trying to self-assemble the shape will end up either bounded with an ultimately periodic pattern covering arbitrarily large squares. This is established thanks to a new characterization of the productions of systems whose productions have a uniformly bounded treewidth.

==> cacarpet.tex <==
\matrix[column sep=3em, nodes={anchor=center}] {
%  \node {$K^0 = \{\vec{0}\}$}; & \node[draw, minimum size=.5cm] {};\\
  \node {$K = K^1 = \kappa(K^0)$}; & \drawcacarpet{1}\\
  \node {$\kappa(\{\vec{0}, \vec{0} + E\})$}; & %
  \begin{scope}
    \drawcacarpet{1}
    \scoped[shift={(1,0)}]{\drawcacarpet{1}}
  \end{scope}\\
    
  \node {$K^2 = \kappa(K^1)$}; & \scoped[scale=3]{\drawcacarpet{2}}\\
%  \node {$K^3 = \kappa(K^2)$}; & \scoped[scale=4]{\drawcacarpet{3}};\\
};

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tikz/cacarpet2.tex <==
\begin{scope}[scale=6]
\drawcacarpet{2};
\end{scope}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.stacs"
%%% End:


==> tikz/empty_gate_EW.tex <==
\node[gate, anchor=center] (gEW) { };
\drawinputEw[1]{(gEW)}
\drawinputWe[0]{(gEW)}

==> tikz/empty_gate_NS.tex <==
\node[gate, anchor=center] (gNS) { };
\drawinputNs[1]{(gNS)}
\drawinputSn[0]{(gNS)}

==> tikz/empty_gate_SE.tex <==
\node[gate, anchor=center] (gSE) { };
\drawinputE{gE}

==> tikz/empty_gate_SW.tex <==
\node[gate, anchor=center] (gSW) { };
\scoped[every path/.style={double}]{\drawinputsW[0]{(gSW)}}
\drawinputSw[1]{(gSW)}
\scoped[draw=green!50!black, very thick, densely dotted]{\drawoutputnE[\footnotesize $1:(E, \{W, N\})$]{(gSW)}}
\scoped[draw=red, very thick, densely dotted]{\drawoutputN[{\footnotesize $0:(N, \{S\})$}]{(gSW)}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.stacs"
%%% End:


==> tikz/empty_gate_SW_sim.tex <==
\node[gate, anchor=center, draw=pink] (gSWsim) { };
\scoped[every path/.style={double}]{\drawinputSw[0]{(gSWsim)}}
\drawinputsW[1]{(gSWsim)}
\scoped[draw=green!50!black]{\drawoutputnE[0]{(gSWsim)}}
\scoped[draw=red, every path/.style={double}]{\drawoutputN[1]{(gSWsim)}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.stacs"
%%% End:


==> tikz/global_input2.tex <==
\begin{scope}[yshift=-2.5cm, xshift=-2.5cm, arrows=-{Stealth}, node font=\small]
  \foreach \x in {0, ..., 5}
  \foreach \y in {0, ..., 5}
  {
    \ifthenelse{\numexpr\(\x=3\and\y=3\)\OR\(\x=2\and\y=2\)\OR\(\x=3\AND\y=2\)\OR\(\x=2\AND\y=3\)}
    {
      
    }%
    {
      \ifthenelse{\numexpr\x=0\and\y=0}{
        \node[gate, draw=red] (gSW\x\y) at (\x, \y) {$+$};
      }{
        \ifthenelse{\numexpr\x=1\and\y=1}{
          \node[gate] (gSW\x\y) at (\x, \y) {$f$};
        }{
          \ifthenelse{\numexpr\(\x=2\and\y=5\)\OR\(\x=5\and\y=4\)}{
            \node[gate, double] (gSW\x\y) at (\x, \y) {$i$};
          }{
            \ifthenelse{\numexpr\x=2\and\y=0}
            {
              \node[gate] (gSW\x\y) at (\x, \y) {$c$};
            }{
              \node[gate] (gSW\x\y) at (\x, \y) {$i$};
            }
          }
        }
      }
    }
  }

  
  \node at (-0.4, -0.2) {0};
  \node at (-0.2, -0.4) {1};
  \node at (-0.45, 0.3) {0};
  \node at (0.2, -0.5) {1};

  \node at (0.55, 0.85) {0};
  \node at (0.85, 0.5) {1};
  \node at (0.8, 1.5) {$n$};
  \node at (1.4, 0.8) {$e$};

  \node at (5.2, 3.6) {0};
  \node at (4.6, 3.9) {1};
  \node at (4.8, 4.4) {0};
  \node at (5.4, 4) {1};
  
  \node at (2.5, 5.1) {0};
  \node at (2.2, 4.5) {1};
  \node at (2.2, 5.5) {1};
  \node at (1.6, 5.2) {0};

  \node at (3.5, 3.9) {0};
  \node at (4.4, 3.9) {0};
  \node at (3.9, 3.6) {1};

  \node at (-0.2, 0.6) {0};
  \node at (-0.4, 0.8) {1};
  \node at (0.4, 0.8) {1};

  
  \node at (0.6, -0.2) {0};
  \node at (0.8, -0.4) {1};
  \node at (0.65, 0.15) {1};
  \node at (1.35, 0.2) {0};


  \drawinputsW[0]{(gSW00)}
  \drawinputSw[2]{(gSW00)}
  \drawinputSw[3]{(gSW10)}
  \drawinputsW[1]{(gSW01)}
  
  \draw (gSW00) .. controls +(-.5, .5) .. (gSW01);
  \draw (gSW00) .. controls +(.5, -.5) .. (gSW10);

  \draw         (gSW10) .. controls +(-.5, .5) .. (gSW11);
  \draw (gSW01) .. controls +( .5, -.5) .. (gSW11);
  \draw (gSW10) .. controls +( .5,  .5) .. (gSW20);
  \draw         (gSW21) .. controls +(-.5, -.5) .. (gSW20);
  

  \foreach \x [evaluate=\x as \xx using \numexpr\x+1] in {2, ..., 4} {
    \draw (gSW\x0) -- (gSW\xx0);
  }

  \foreach \x [evaluate=\x as \xx using \numexpr\x+1] in {1, ..., 3} {
    \draw (gSW\x1) -- (gSW\xx1);
    \ifthenelse{\x=3}
    {
      \draw (gSW\x4) ..controls +(.5, -.5) .. (gSW\xx4);
    }{
      \draw (gSW\x4) -- (gSW\xx4);
    }

  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y+1] in {1, ..., 3} {
    \draw (gSW1\y) -- (gSW1\yy);
    \ifthenelse{\y=3}
    {
      \draw (gSW4\y) ..controls +(-.5, .5) .. (gSW4\yy);
    }{
      \draw (gSW4\y) -- (gSW4\yy);
    }
  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y+1] in {0, ..., 4} {
    \draw (gSW5\y) -- (gSW5\yy);
  }

  \foreach \x [evaluate=\x as \xx using \numexpr\x-1] in {1, ..., 5} {
    \draw (gSW\x5) -- (gSW\xx5);
  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y-1] in {3, ..., 5} {
    \draw (gSW0\y) -- (gSW0\yy);
  }
  

  \scoped[draw=red, every path/.style={double, densely dotted}]{\drawoutputN[0]{(gSW35)}}
  \scoped[draw=red, densely dotted]{\drawoutputNe[1]{(gSW25)}}
  \draw[draw=red, double, densely dotted] (gSW35) .. controls +(-.5, -.5) .. (gSW25);
  \draw[draw=red, densely dotted] (gSW24) .. controls +(.5, .5) .. (gSW25);

  \scoped[draw=green!50!black, every path/.style={double, densely dotted}]{\drawoutputnE[2]{(gSW55)}}
  \scoped[draw=green!50!black, densely dotted]{\drawoutputnE[3]{(gSW54)}}
  \draw[draw=green!50!black, densely dotted] (gSW44) .. controls +(.5, -.5) .. (gSW54);
  \draw[draw=green!50!black, double, densely dotted] (gSW53) .. controls +(-.5, .5) .. (gSW54);

  
  % \scoped[draw=blue!50!black, every path/.style={double, densely dotted}]{\drawoutputSe{(gE50)}}
  % \scoped[draw=blue!50!black, densely dotted]{\drawoutputSe{(gE40)}}
  % \draw[draw=blue!50!black, densely dotted] (gE41) .. controls +(.5, -.5) .. (gE40);
  % \draw[draw=blue!50!black, double, densely dotted] (gE50) .. controls +(-.5, .5) .. (gE40);


\end{scope}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.stacs"
%%% End:


==> tikz/global_normal1.tex <==
\begin{scope}[yshift=-2.5cm, xshift=-2.5cm, arrows=-{Stealth}, node font=\small]
  \foreach \x in {0, ..., 5}
  \foreach \y in {0, ..., 5}
  {
    \ifthenelse{\numexpr\(\x=3\and\y=3\)\OR\(\x=2\and\y=2\)\OR\(\x=3\AND\y=2\)\OR\(\x=2\AND\y=3\)}
    {
      
    }%
    {
      \ifthenelse{\numexpr\x=5\and\y=3}{
        \node[gate] (gE\x\y) at (\x, \y) {$+$};
      }{
        \ifthenelse{\numexpr\x=5\and\y=2}{
          \node[gate, fill=yellow] (gE\x\y) at (\x, \y) {$*$};
        }
        {
          \ifthenelse{\numexpr\x=4\and\y=0}{
            \node[gate, double] (gE\x\y) at (\x, \y) {$i$};
          }{
            \ifthenelse{\numexpr\x=0\and\y=4}{
              \node[gate, double] (gE\x\y) at (\x, \y) {$i$};
            }{
              \ifthenelse{\numexpr\x=2\and\y=5}{
                \node[gate, double] (gE\x\y) at (\x, \y) {$i$};
              }{
                \node[gate] (gE\x\y) at (\x, \y) {$i$};
              }
            }
          }
        }
      }
    }
  }

  \node at (4.4, -0.2) {0};
  \node at (3.6, -0.2) {0};
  \node at (4.1, -0.5) {1};
  \node at (4.1, 0.5) {1};

  \node at (-0.4, 3.8) {1};
  \node at (0.4, 4) {1};
  \node at (0.1, 4.4) {0};
  \node at (0.1, 3.5) {0};

  \node at (2.4, 4.8) {0};
  \node at (1.6, 5.3) {0};
  \node at (2.1, 5.5) {1};
  \node at (1.8, 4.6) {1};
  
  \scoped{\drawinputE[0]{(gE53)}}
  \drawinputEn[1]{(gE52)}
  \draw (gE53) .. controls +(.5, -.5) .. (gE52);
  \draw (gE52) -- (gE51);
  \draw (gE51) -- (gE50);
  \draw (gE55) -- (gE54);
  \draw (gE52) -- (gE42);

  \foreach \x [evaluate=\x as \xx using \numexpr\x+1] in {0, ..., 4} {
    \ifthenelse{\numexpr\x=4}
    {
      \draw[double, densely dotted] (gE\xx0) -- (gE\x0);
    }{
      \draw (gE\xx0) -- (gE\x0);
    }
  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y-1] in {1, ..., 5} {
    \ifthenelse{\numexpr\y=4}
    {
      \draw[double, densely dotted] (gE0\yy) -- (gE0\y);
    }
    {
      \draw (gE0\yy) -- (gE0\y);
    }
    \ifthenelse{\numexpr\y=2}
    {
      \draw[double, densely dotted] (gE\yy5) -- (gE\y5);
    }{
      \draw (gE\yy5) -- (gE\y5);
    }
  }


  \draw (gE42) -- (gE43);
  \draw (gE43) -- (gE44);

  \foreach \k [evaluate=\k as \kk using \numexpr\k+1] in {3, 2, 1} {
    \draw (gE\kk4) -- (gE\k4);
    \draw (gE1\kk) -- (gE1\k);
  }

  \foreach \x [evaluate=\x as \xx using \numexpr\x-1] in {2, 3, 4} {
    \draw (gE\xx1) -- (gE\x1);
  }

  \scoped[draw=red, every path/.style={densely dotted}]{\drawoutputN[0]{(gE35)}}
  \scoped[draw=red, densely dotted]{\drawoutputNe[1]{(gE25)}}
  \draw[draw=red, densely dotted] (gE15) .. controls +(.5, -.5) .. (gE25);
  \draw[draw=red, densely dotted] (gE24) .. controls +(-.5, .5) .. (gE25);

  \scoped[draw=green!50!black, every path/.style={densely dotted}]{\drawoutputnW[2]{(gE05)}}
  \scoped[draw=green!50!black, densely dotted]{\drawoutputnW[3]{(gE04)}}
  \draw[draw=green!50!black, densely dotted] (gE14) .. controls +(-.5, -.5) .. (gE04);
  \draw[draw=green!50!black, densely dotted] (gE03) .. controls +(.5, .5) .. (gE04);

  
  \scoped[draw=blue!50!black, every path/.style={densely dotted}]{\drawoutputSe[4]{(gE50)}}
  \scoped[draw=blue!50!black, densely dotted]{\drawoutputSe[5]{(gE40)}}
  \draw[draw=blue!50!black, densely dotted] (gE41) .. controls +(.5, -.5) .. (gE40);
  \draw[draw=blue!50!black, densely dotted] (gE50) .. controls +(-.5, .5) .. (gE40);


\end{scope}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.stacs"
%%% End:


==> tikz/global_normal2.tex <==
\begin{scope}[yshift=-2.5cm, xshift=-2.5cm, arrows=-{Stealth}, node font=\small]
  \foreach \x in {0, ..., 5}
  \foreach \y in {0, ..., 5}
  {
    \ifthenelse{\numexpr\(\x=3\and\y=3\)\OR\(\x=2\and\y=2\)\OR\(\x=3\AND\y=2\)\OR\(\x=2\AND\y=3\)}
    {
      
    }%
    {
      \ifthenelse{\numexpr\x=0\and\y=0}{
        \node[gate, draw=red] (gSW\x\y) at (\x, \y) {$+$};
      }{
        \ifthenelse{\numexpr\x=1\and\y=1}{
          \node[gate] (gSW\x\y) at (\x, \y) {$f$};
        }{
          \ifthenelse{\numexpr\(\x=2\and\y=5\)\OR\(\x=5\and\y=4\)}{
            \node[gate, double] (gSW\x\y) at (\x, \y) {$i$};
          }{
            \node[gate] (gSW\x\y) at (\x, \y) {$i$};
          }
        }
      }
    }
  }

  \node at (-0.4, -0.2) {0};
  \node at (-0.2, -0.4) {1};
  \node at (-0.45, 0.3) {0};
  \node at (0.2, -0.5) {1};

  \node at (0.55, 0.85) {0};
  \node at (0.85, 0.5) {1};
  \node at (0.8, 1.5) {$n$};
  \node at (1.4, 0.8) {$e$};

  \node at (5.2, 3.6) {0};
  \node at (4.6, 3.9) {1};
  \node at (4.8, 4.4) {0};
  \node at (5.4, 4) {1};
  
  \node at (2.5, 5.1) {0};
  \node at (2.2, 4.5) {1};
  \node at (2.2, 5.5) {1};
  \node at (1.6, 5.2) {0};

  \node at (3.5, 3.9) {0};
  \node at (4.4, 3.9) {0};
  \node at (3.9, 3.6) {1};

  \node at (-0.2, 0.6) {0};
  \node at (-0.4, 0.8) {1};
  \node at (0.4, 0.8) {1};

  
  \node at (0.6, -0.2) {0};
  \node at (0.8, -0.4) {1};
  \node at (0.65, 0.15) {1};
  \node at (1.35, 0.2) {0};
  
  \drawinputsW[0]{(gSW00)}
  \drawinputsW[1]{(gSW01)}
  \drawinputSw[2]{(gSW00)}
  \drawinputSw[3]{(gSW10)}

  
  \draw (gSW00) .. controls +(-.5, .5) .. (gSW01);
  \draw (gSW00) .. controls +(.5, -.5) .. (gSW10);

  \draw (gSW10) .. controls +(-.5, .5) .. (gSW11);
  \draw (gSW01) .. controls +(.5, -.5) .. (gSW11);

  \foreach \x [evaluate=\x as \xx using \numexpr\x+1] in {1, ..., 4} {
    \draw (gSW\x0) -- (gSW\xx0);
  }

  \foreach \x [evaluate=\x as \xx using \numexpr\x+1] in {1, ..., 3} {
    \draw (gSW\x1) -- (gSW\xx1);
    \ifthenelse{\x=3}
    {
      \draw (gSW\x4) ..controls +(.5, -.5) .. (gSW\xx4);
    }{
      \draw (gSW\x4) -- (gSW\xx4);
    }

  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y+1] in {1, ..., 3} {
    \draw (gSW1\y) -- (gSW1\yy);
    \ifthenelse{\y=3}
    {
      \draw (gSW4\y) ..controls +(-.5, .5) .. (gSW4\yy);
    }{
      \draw (gSW4\y) -- (gSW4\yy);
    }
  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y+1] in {0, ..., 4} {
    \draw (gSW5\y) -- (gSW5\yy);
  }

  \foreach \x [evaluate=\x as \xx using \numexpr\x-1] in {1, ..., 5} {
    \draw (gSW\x5) -- (gSW\xx5);
  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y-1] in {3, ..., 5} {
    \draw (gSW0\y) -- (gSW0\yy);
  }
  

  \scoped[draw=red, every path/.style={double, densely dotted}]{\drawoutputN[$n$]{(gSW35)}}
  \scoped[draw=red, densely dotted]{\drawoutputNe[$n+1$]{(gSW25)}}
  \draw[draw=red, double, densely dotted] (gSW35) .. controls +(-.5, -.5) .. (gSW25);
  \draw[draw=red, densely dotted] (gSW24) .. controls +(.5, .5) .. (gSW25);

  \scoped[draw=green!50!black, every path/.style={double, densely dotted}]{\drawoutputnE[$e$]{(gSW55)}}
  \scoped[draw=green!50!black, densely dotted]{\drawoutputnE[$e+1$]{(gSW54)}}
  \draw[draw=green!50!black, densely dotted] (gSW44) .. controls +(.5, -.5) .. (gSW54);
  \draw[draw=green!50!black, double, densely dotted] (gSW53) .. controls +(-.5, .5) .. (gSW54);

  
  % \scoped[draw=blue!50!black, every path/.style={double, densely dotted}]{\drawoutputSe{(gE50)}}
  % \scoped[draw=blue!50!black, densely dotted]{\drawoutputSe{(gE40)}}
  % \draw[draw=blue!50!black, densely dotted] (gE41) .. controls +(.5, -.5) .. (gE40);
  % \draw[draw=blue!50!black, double, densely dotted] (gE50) .. controls +(-.5, .5) .. (gE40);


\end{scope}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.stacs"
%%% End:


==> tikz/global_sim.tex <==
\begin{scope}[yshift=-2.5cm, xshift=-2.5cm, arrows=-{Stealth}, node font=\small]
  \foreach \x in {0, ..., 5}
  \foreach \y in {0, ..., 5}
    {
    \ifthenelse{\numexpr\(\x=3\and\y=3\)\OR\(\x=2\and\y=2\)\OR\(\x=3\AND\y=2\)\OR\(\x=2\AND\y=3\)}
    {
      
    }%
    {
      \ifthenelse{\numexpr\x=0\and\y=0}{
        \node[gate, draw=red] (gSW\x\y) at (\x, \y) {$+$};
      }{
        \ifthenelse{\numexpr\x=1\and\y=1}{
          \node[gate] (gSW\x\y) at (\x, \y) {$f$};
        }{
          \ifthenelse{\numexpr\(\x=2\and\y=5\)\OR\(\x=5\and\y=4\)}{
            \node[gate, double] (gSW\x\y) at (\x, \y) {$i$};
          }{
            \node[gate] (gSW\x\y) at (\x, \y) {$i$};
          }
        }
      }
    }
  }

  \scoped[every path/.style={double}]{\drawinputSw[0]{(gSW00)}}
  \drawinputsW[2]{(gSW00)}
  \drawinputSw[1]{(gSW10)}
  \drawinputsW[3]{(gSW01)}
  
  \draw[double] (gSW00) .. controls +(-.5, .5) .. (gSW01);
  \draw[double] (gSW00) .. controls +(.5, -.5) .. (gSW10);

  \draw (gSW10) .. controls +(-.5, .5) .. (gSW11);
  \draw[double] (gSW01) .. controls +(.5, -.5) .. (gSW11);

  \foreach \x [evaluate=\x as \xx using \numexpr\x+1] in {1, ..., 4} {
    \draw[double] (gSW0\x) -- (gSW0\xx);
  }

  \foreach \x [evaluate=\x as \xx using \numexpr\x+1] in {1, ..., 3} {
    \draw[double] (gSW\x1) -- (gSW\xx1);
    \ifthenelse{\x=3}
    {
      \draw (gSW\x4) ..controls +(.5, -.5) .. (gSW\xx4);
    }{
      \draw[double] (gSW\x4) -- (gSW\xx4);
    }

  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y+1] in {1, ..., 3} {
    \draw[double] (gSW1\y) -- (gSW1\yy);
    \ifthenelse{\y=3}
    {
      \draw[double] (gSW4\y) ..controls +(-.5, .5) .. (gSW4\yy);
    }{
      \draw[double] (gSW4\y) -- (gSW4\yy);
    }
  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y+1] in {0, ..., 4} {
    \draw[double] (gSW\y5) -- (gSW\yy5);
  }

  \foreach \x [evaluate=\x as \xx using \numexpr\x-1] in {1, ..., 5} {
    \draw[double] (gSW5\x) -- (gSW5\xx);
  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y-1] in {3, ..., 5} {
    \draw[double] (gSW\y0) -- (gSW\yy0);
  }
  

  \scoped[draw=red, every path/.style={double, densely dotted}]{\drawoutputN[2]{(gSW35)}}
  \scoped[draw=red, densely dotted]{\drawoutputNe[3]{(gSW25)}}
  \draw[draw=red, double, densely dotted] (gSW35) .. controls +(-.5, -.5) .. (gSW25);
  \draw[draw=red, densely dotted] (gSW24) .. controls +(.5, .5) .. (gSW25);

  \scoped[draw=green!50!black, every path/.style={double, densely dotted}]{\drawoutputnE[0]{(gSW55)}}
  \scoped[draw=green!50!black, densely dotted]{\drawoutputnE[1]{(gSW54)}}
  \draw[draw=green!50!black, densely dotted] (gSW44) .. controls +(.5, -.5) .. (gSW54);
  \draw[draw=green!50!black, double, densely dotted] (gSW53) .. controls +(-.5, .5) .. (gSW54);

  
  % \scoped[draw=blue!50!black, every path/.style={double, densely dotted}]{\drawoutputSe{(gE50)}}
  % \scoped[draw=blue!50!black, densely dotted]{\drawoutputSe{(gE40)}}
  % \draw[draw=blue!50!black, densely dotted] (gE41) .. controls +(.5, -.5) .. (gE40);
  % \draw[draw=blue!50!black, double, densely dotted] (gE50) .. controls +(-.5, .5) .. (gE40);


\end{scope}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.stacs"
%%% End:


==> tikz/headroom.tex <==
\makeatletter
\pgfarrowsdeclare{...}{...}{%
  \pgfutil@tempdima\pgflinewidth
  \pgfarrowsrightextend{+6.5\pgfutil@tempdima}%
  \pgfarrowsleftextend{+6.5\pgfutil@tempdima}%
}{
  \pgfutil@tempdima\pgflinewidth
  \pgfpathcircle{\pgfqpoint{+4\pgfutil@tempdima}{+0pt}}{+.8\pgfutil@tempdima}%
  \pgfpathcircle{\pgfqpoint{+8\pgfutil@tempdima}{+0pt}}{+.8\pgfutil@tempdima}%
  \pgfpathcircle{\pgfqpoint{+12\pgfutil@tempdima}{+0pt}}{+.8\pgfutil@tempdima}%
  \pgfusepathqfill
}
\makeatother

\def\StairData{%
1 0 0 0
1 1 0 1
1 1 1 1
}
\readarray\StairData\Stair[-,4]

\fractalify{2}{\Stair}{\StairCOLS}{\StairROWS}

\foreach \y in {5, 6, 7, 8}
\filldraw[fill=gray!20] (0, \y) -- ++(1,0) -- ++(0,1) -- ++(-1,0) -- cycle;

\filldraw[fill=gray!20] (8, 8) -- ++(1,0) -- ++(0,1) -- ++(-1,0) -- cycle;
\filldraw[fill=gray!20] (3, 7) -- ++(1,0) -- ++(0,1) -- ++(-1,0) -- cycle;

\foreach \y [count=\column,remember=\y as \lasty (initially 0), remember=\column as \lastcol (initially 0)]%
in {0, 1, 2, 1, 3, 4, 5, 4, 6, 7, 8, 7, 3, 4, 5, 4, 9}
\draw[red, ultra thick] (\lastcol, \lasty) -- (\lastcol, \y) -- (\column, \y);

\node[red, anchor=west] at (17, 9) {$x \mapsto \theFloor(x)$};



\foreach \x / \y [remember=\x as \lastx (initially -.4), remember=\y as \lasty (initially 1)]%
in {0/1, 0/5, 1/5, 1/6, 4/6, 4/8, 2/8, 2/7, 1/7, 1/9, 8/9, 8/8, 9/8, 9/9, 11/9, 11/10}
\draw[purple, ultra thick] (\lastx, \lasty) -- (\x, \y);

\node[purple, anchor=south] at (11, 10) {$\ell P$};


\begin{scope}[blue]
  \foreach \x / \ymin / \ymax [count=\c, remember=\x as \lastx] in {0/0/1, 8/6/8, 9/7/9, 10/8/9, 11/8/9} {
    \pgfmathsetmacro\actualc{int(\c - 1)}
    \pgfmathsetmacro\prevc{int(\actualc - 1)}
    \pgfmathsetmacro\ynode{.5*mod(\c, 2)-3.5}
    \pgfmathsetmacro\yarrow{mod(\c, 2)-1.5}
    \pgfmathsetmacro\arrownodepos{ (\prevc ==  2 || \prevc == 1) ? "below" : "above"}
    \node (t\c) at (\x, \ynode) {$t_{\actualc}(2, P)$};
    \draw[ultra thick] (\x, \ymin) -- (\x, \ymax);
    \draw[dashed, on background layer] (\x, \ymin) -- (t\c);
    \ifthenelse{\numexpr\c>1}{
      \draw (\lastx, \yarrow) edge[<->] node[\arrownodepos, fill=white, outer sep=3pt]{$\wexcursion(2, P, \prevc)$} (\x, \yarrow);
    }{}
  }
  \draw (11, 1) edge[<-...] node[above]{$\wexcursion(2, P, 5)$} (17, 1);
\end{scope}

\draw[thick, shift={(.5, 0)}] (1, 1) edge[<->] node[fill=white, rounded corners, pos=.70] {$\altitude(2, P, 0)$} (1, 9);
\draw[thick, shift={(.5, 0)}] (0, 0) edge[<->] node[fill=white, rounded corners] {$\headroom[P](0)$} (0, 5);
\draw[thick, shift={(.5, 0)}] (3, 1) edge[<->] node[fill=white, rounded corners] {$\headroom[P](3)$} (3, 6);
\draw[thick, shift={(.5, 0)}] (8, 6) edge[<->] node[fill=white, rounded corners] {$\headroom[P](8)$} (8, 8);


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "standalone"
%%% End:


==> tikz/in_out_wires_E_N_Nw_Se.tex <==
\begin{scope}[scale=.6,yshift=-2.5cm, xshift=-2.5cm]
  \foreach \x in {0, ..., 5}
  \foreach \y in {0, ..., 5}
  {
    \ifthenelse{\numexpr\(\x=3\and\y=3\)\OR\(\x=2\and\y=2\)\OR\(\x=3\AND\y=2\)\OR\(\x=2\AND\y=3\)}
    {
      
    }%
    {
      \node[gate, inner sep=.5mm, fill=black] (gE\x\y) at (\x, \y) { };
    }
  }
  \drawinputE{gE53}
  \drawinputEs{gE52}
\end{scope}


==> tikz/local_nondet_pat.tex <==

\begin{scope}[scale=1.5,val1/.style={fill=red}]
  \foreach \x in {1, ..., 5}
  \foreach \y in {1, ..., 5}{
    % \ifthenelse{\or{\or{\equal{\z}{1}}{\equal{\x}{1}}}{\equal{\y}{1}}}{
      \node[draw, circle] (n\x\y) at (\x, \y) {\Sierp[\x,\y]};
      % }{
      %\node[draw, circle, fill=gray!25] (n\x\y) at (\x, \y) {\Sierp[\x,\y]};
      % }
  }
    
  \foreach \x in {1, ..., 5} {
    \node (n\x6) at (\x, 6) {...};
    \node (n6\x) at (6, \x) {...};
  }
\end{scope}

\foreach \y [evaluate=\y as \yy using \numexpr\y+1] in {1, ..., 5}
\foreach \x in {1, ..., 5} {
  \ifthenelse{\numexpr\x=1}{
    \draw (n\x\y)  edge[->] node [fill=gray!50] {A} (n\x\yy);
    \draw (n\y\x)  edge[->] node [fill=gray!50] {A} (n\yy\x);
  } {
    \ifthenelse{\numexpr\z=1} {
      \draw (n\x\y)  edge[->] node (a\x\y) [fill=blue!50] {\z} (n\x\yy);
      \draw (n\y\x)  edge[->] node (a\y\x) [fill=blue!50] {\z} (n\yy\x);
    }
  }
}

\draw[red, thick] (a32) circle [radius=.5];
\draw[red, thick] (a13) circle [radius=.5];

% \node[red] at (5, 6) {0 0 \Sierp(1, 1)};
% \node[green] at (6, 6) {0 1 \Sierp(1, 2)};
% \node[blue] at (5, 7) {1 0 \Sierp(2, 1)};
% %\node[draw, rectangle,xshift=5cm] at (\x, \y) {\x \y \yy};

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.stacs"
%%% End:


==> tikz/local_normal2.tex <==
\begin{scope}[yshift=-2.5cm, xshift=-2.5cm, arrows=-{Stealth}, node font=\small]
  \foreach \x in {0, ..., 5}
  \foreach \y in {0, ..., 5}
  {
    \ifthenelse{\numexpr\(\x=3\and\y=3\)\OR\(\x=2\and\y=2\)\OR\(\x=3\AND\y=2\)\OR\(\x=2\AND\y=3\)}
    {
      
    }%
    {
      \ifthenelse{\numexpr\x=0\and\y=0}{
        \node[gate, draw=red] (gSW\x\y) at (\x, \y) {$p$};
      }{
        \node[gate] (gSW\x\y) at (\x, \y) {$i$};
      }
    }
  }

  \scoped[every path/.style={double}]{\drawinputsW[0]{(gSW00)}}
  \drawinputSw[2]{(gSW00)}
  \drawinputSw[3]{(gSW10)}
  \drawinputsW[1]{(gSW01)}
  
  \draw[double] (gSW00) .. controls +(-.5, .5) .. (gSW01);
  \draw[double] (gSW00) .. controls +(.5, -.5) .. (gSW10);

  \draw (gSW10) .. controls +(-.5, .5) .. (gSW11);
  \draw[double] (gSW01) .. controls +(.5, -.5) .. (gSW11);

  \foreach \x [evaluate=\x as \xx using \numexpr\x+1] in {1, ..., 4} {
    \draw[double] (gSW\x0) -- (gSW\xx0);
  }

  \foreach \x [evaluate=\x as \xx using \numexpr\x+1] in {1, ..., 3} {
    \draw[double] (gSW\x1) -- (gSW\xx1);
    \ifthenelse{\x=3}
    {
      \draw (gSW\x4) ..controls +(.5, -.5) .. (gSW\xx4);
    }{
      \draw[double] (gSW\x4) -- (gSW\xx4);
    }

  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y+1] in {1, ..., 3} {
    \draw[double] (gSW1\y) -- (gSW1\yy);
    \ifthenelse{\y=3}
    {
      \draw[double] (gSW4\y) ..controls +(-.5, .5) .. (gSW4\yy);
    }{
      \draw[double] (gSW4\y) -- (gSW4\yy);
    }
  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y+1] in {0, ..., 4} {
    \draw[double] (gSW5\y) -- (gSW5\yy);
  }

  \foreach \x [evaluate=\x as \xx using \numexpr\x-1] in {1, ..., 5} {
    \draw[double] (gSW\x5) -- (gSW\xx5);
  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y-1] in {3, ..., 5} {
    \draw[double] (gSW0\y) -- (gSW0\yy);
  }
  

  \scoped[draw=red, every path/.style={double, densely dotted}]{\drawoutputN[0]{(gSW35)}}
  \scoped[draw=red, densely dotted]{\drawoutputNe[1]{(gSW25)}}
  \draw[draw=red, double, densely dotted] (gSW35) .. controls +(-.5, -.5) .. (gSW25);
  \draw[draw=red, densely dotted] (gSW24) .. controls +(.5, .5) .. (gSW25);

  \scoped[draw=green!50!black, every path/.style={double, densely dotted}]{\drawoutputnE[2]{(gSW55)}}
  \scoped[draw=green!50!black, densely dotted]{\drawoutputnE[3]{(gSW54)}}
  \draw[draw=green!50!black, densely dotted] (gSW44) .. controls +(.5, -.5) .. (gSW54);
  \draw[draw=green!50!black, double, densely dotted] (gSW53) .. controls +(-.5, .5) .. (gSW54);

  
  % \scoped[draw=blue!50!black, every path/.style={double, densely dotted}]{\drawoutputSe{(gE50)}}
  % \scoped[draw=blue!50!black, densely dotted]{\drawoutputSe{(gE40)}}
  % \draw[draw=blue!50!black, densely dotted] (gE41) .. controls +(.5, -.5) .. (gE40);
  % \draw[draw=blue!50!black, double, densely dotted] (gE50) .. controls +(-.5, .5) .. (gE40);


\end{scope}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.stacs"
%%% End:


==> tikz/local_sim.tex <==
\begin{scope}[yshift=-2.5cm, xshift=-2.5cm, arrows=-{Stealth}, node font=\small]
  \foreach \x in {0, ..., 5}
  \foreach \y in {0, ..., 5}
  {
    \ifthenelse{\numexpr\(\x=3\and\y=3\)\OR\(\x=2\and\y=2\)\OR\(\x=3\AND\y=2\)\OR\(\x=2\AND\y=3\)}
    {
      
    }%
    {
      \ifthenelse{\numexpr\x=0\and\y=0}{
        \node[gate, draw=red] (gSW\x\y) at (\x, \y) {$p$};
      }{
        \node[gate] (gSW\x\y) at (\x, \y) {$i$};
      }
    }
  }

  \scoped[every path/.style={double}]{\drawinputSw[0]{(gSW00)}}
  \drawinputsW[2]{(gSW00)}
  \drawinputSw[1]{(gSW10)}
  \drawinputsW[3]{(gSW01)}
  
  \draw[double] (gSW00) .. controls +(-.5, .5) .. (gSW01);
  \draw[double] (gSW00) .. controls +(.5, -.5) .. (gSW10);

  \draw (gSW10) .. controls +(-.5, .5) .. (gSW11);
  \draw[double] (gSW01) .. controls +(.5, -.5) .. (gSW11);

  \foreach \x [evaluate=\x as \xx using \numexpr\x+1] in {1, ..., 4} {
    \draw[double] (gSW0\x) -- (gSW0\xx);
  }

  \foreach \x [evaluate=\x as \xx using \numexpr\x+1] in {1, ..., 3} {
    \draw[double] (gSW\x1) -- (gSW\xx1);
    \ifthenelse{\x=3}
    {
      \draw (gSW\x4) ..controls +(.5, -.5) .. (gSW\xx4);
    }{
      \draw[double] (gSW\x4) -- (gSW\xx4);
    }

  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y+1] in {1, ..., 3} {
    \draw[double] (gSW1\y) -- (gSW1\yy);
    \ifthenelse{\y=3}
    {
      \draw[double] (gSW4\y) ..controls +(-.5, .5) .. (gSW4\yy);
    }{
      \draw[double] (gSW4\y) -- (gSW4\yy);
    }
  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y+1] in {0, ..., 4} {
    \draw[double] (gSW\y5) -- (gSW\yy5);
  }

  \foreach \x [evaluate=\x as \xx using \numexpr\x-1] in {1, ..., 5} {
    \draw[double] (gSW5\x) -- (gSW5\xx);
  }

  \foreach \y [evaluate=\y as \yy using \numexpr\y-1] in {3, ..., 5} {
    \draw[double] (gSW\y0) -- (gSW\yy0);
  }
  

  \scoped[draw=red, every path/.style={double, densely dotted}]{\drawoutputN[2]{(gSW35)}}
  \scoped[draw=red, densely dotted]{\drawoutputNe[3]{(gSW25)}}
  \draw[draw=red, double, densely dotted] (gSW35) .. controls +(-.5, -.5) .. (gSW25);
  \draw[draw=red, densely dotted] (gSW24) .. controls +(.5, .5) .. (gSW25);

  \scoped[draw=green!50!black, every path/.style={double, densely dotted}]{\drawoutputnE[0]{(gSW55)}}
  \scoped[draw=green!50!black, densely dotted]{\drawoutputnE[1]{(gSW54)}}
  \draw[draw=green!50!black, densely dotted] (gSW44) .. controls +(.5, -.5) .. (gSW54);
  \draw[draw=green!50!black, double, densely dotted] (gSW53) .. controls +(-.5, .5) .. (gSW54);

  
  % \scoped[draw=blue!50!black, every path/.style={double, densely dotted}]{\drawoutputSe{(gE50)}}
  % \scoped[draw=blue!50!black, densely dotted]{\drawoutputSe{(gE40)}}
  % \draw[draw=blue!50!black, densely dotted] (gE41) .. controls +(.5, -.5) .. (gE40);
  % \draw[draw=blue!50!black, double, densely dotted] (gE50) .. controls +(-.5, .5) .. (gE40);


\end{scope}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.stacs"
%%% End:


==> tikz/seed_global.tex <==
\begin{scope}[arrows=-{Stealth}]
  \foreach \x in {0, ..., 5}
  \foreach \y in {0, ..., 5}
  {
    \ifthenelse{\numexpr\(\x=3\and\y=3\)\OR\(\x=2\and\y=2\)\OR\(\x=3\AND\y=2\)\OR\(\x=2\AND\y=3\)}
    {
      
    }%
    {
      \ifthenelse{\numexpr\x=0\AND\y=0}{
        \node[gate, inner sep=.5mm, fill=red] (s\x\y) at (\x, \y) { $s$ };
      }%
      {
        \ifthenelse{\numexpr\x=5\AND\y=3}{
          \node[gate, inner sep=.5mm] (s\x\y) at (\x, \y) { $i_2$ };
        }%
        {
          \node[gate, inner sep=.5mm] (s\x\y) at (\x, \y) { $i_1$ };
        }
      }
    }
  }
  \draw (s43) .. controls +(.5, -.5) .. (s53) node[pos=.9, auto=left] {\footnotesize $1$} ;
  \pgfkeys{/pgf/number format/.cd,int detect,precision=2}
  \foreach \x [evaluate=\x as \xx using \numexpr\x-1] in {1, ..., 5} {
    \draw (s\xx0) -- (s\x0);
    \ifthenelse{\x=3}{
      \draw (s5\xx) .. controls +(-.5,.5) .. (s5\x) node[pos=.9, auto=right] {\footnotesize $0$};
    }{
      \ifthenelse{\x=4}{
        \draw (s5\xx) -- (s5\x) node[pos=.1, auto=right, node font=\footnotesize] {$0$};
      }{
        \draw (s5\xx) -- (s5\x);
      }
    }
    \ifthenelse{\numexpr\x<5\and\xx>0}{
      \draw (s1\xx) -- (s1\x);
      \draw (s\xx4) -- (s\x4);
    }{}
  }
  
  \foreach \x  [evaluate=\x as \xx using \numexpr\x+1] in {4, 3, ..., 0} {
    \draw (s\xx5) -- (s\x5);
    \ifthenelse{\numexpr\x>0}{
      \draw (s0\xx) -- (s0\x);
    }{}
    \ifthenelse{\numexpr\x>0\and\xx<5}{
      \draw (s4\xx) -- (s4\x);
      \ifthenelse{\numexpr\x>1}{
        \draw (s\xx1) -- (s\x1);
      }{}
    }{}
  }

  \draw (s10) -- (s11);
  \drawoutputE[0]{(s52)}
  \drawoutputsE[1]{(s53)}
\end{scope}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.stacs"
%%% End:

